Position-Indexed Formulations for Kidney Exchange

A kidney exchange is an organized barter market where patients in need of a kidney swap willing but incompatible donors. Determining an optimal set of exchanges is theoretically and empirically hard. Traditionally, exchanges took place in cycles, with each participating patient-donor pair both giving and receiving a kidney. The recent introduction of chains, where a donor without a paired patient triggers a sequence of donations without requiring a kidney in return, increased the efficacy of fielded kidney exchanges---while also dramatically raising the empirical computational hardness of clearing the market in practice. While chains can be quite long, unbounded-length chains are not desirable: planned donations can fail before transplant for a variety of reasons, and the failure of a single donation causes the rest of that chain to fail, so parallel shorter chains are better in practice. In this paper, we address the tractable clearing of kidney exchanges with short cycles and chains that are long but bounded. This corresponds to the practice at most modern fielded kidney exchanges. We introduce three new integer programming formulations, two of which are compact. Furthermore, one of these models has a linear programming relaxation that is exactly as tight as the previous tightest formulation (which was not compact) for instances in which each donor has a paired patient. On real data from the UNOS nationwide exchange in the United States and the NLDKSS nationwide exchange in the United Kingdom, as well as on generated realistic large-scale data, we show that our new models are competitive with all existing solvers---in many cases outperforming all other solvers by orders of magnitude.

==> figs/fig_pief_further_reduction.tex <==
\begin{tikzpicture}[scale=0.8,transform shape]

  \foreach \n in {1, ..., 3} {
    \c=\n
    \multiply\c by 2
    \node[whitecirc] (N\n) at (\the\c, 0) {\n};
  }

  \foreach \m/\n in {1/2, 2/3, 3/2, 2/1}
  \draw[-latex, bend left] (N\m) to node {} (N\n);
\end{tikzpicture}



==> sections/exp_tables/1000pairs_10alts_mean.tex <==
\begin{table}[ht!bp]
\centering
\caption{$|P|~=~1000,~|A|~=~10$}
\begin{tabular}
{ c r | r  | r  | r  | r  | r  | r  | r  | r  | r  | r  | r }
Method & & $L = 2$ & $L = 3$ & $L = 4$ & $L = 5$ & $L = 6$ & $L = 7$ & $L = 8$ & $L = 9$ & $L = 10$ & $L = 11$ & $L = 12$\\
\hline\\\\
$\textsc{BnP-Poly}$ & Mean & $1144.66$& $1148.55$& $2265.22$& $2045.53$& $2499.77$& $2938.63$& $3384.22$& $3409.41$& $3600.15$& $3600.15$& $3600.10$\\
& Stdev & $1242.98$& $1241.74$& $1177.74$& $1647.09$& $852.38$& $854.00$& $571.22$& $504.58$& $0.06$& $0.08$& $0.07$\\
& Min& $27.32$& $27.66$& $37.92$& $41.77$& $1831.69$& $1828.04$& $1872.91$& $2074.42$& $3600.07$& $3600.03$& $3600.03$\\
 & Max& $3600.03$& $3600.03$& $3600.14$& $3600.17$& $3600.23$& $3600.22$& $3600.31$& $3600.33$& $3600.25$& $3600.23$& $3600.22$\\
\hline\\\\
\end{tabular}

\label{tbl:data}
\end{table}

==> sections/exp_tables/300pairs_0alts_mean.tex <==
\begin{table}[ht!bp]
\centering
\caption{$|P|~=~300,~|A|~=~0$}
\begin{tabular}
{ c r | r  | r  | r  | r  | r  | r  | r  | r  | r  | r  | r }
Method & & $L = 2$ & $L = 3$ & $L = 4$ & $L = 5$ & $L = 6$ & $L = 7$ & $L = 8$ & $L = 9$ & $L = 10$ & $L = 11$ & $L = 12$\\
\hline\\\\
$\textsc{PICEF}$ & Mean & $0.69$& $0.70$& $0.70$& $0.72$& $0.74$& $0.73$& $0.74$& $0.76$& $0.77$& $0.78$& $0.78$\\
& Stdev & $0.40$& $0.41$& $0.41$& $0.43$& $0.43$& $0.44$& $0.45$& $0.46$& $0.48$& $0.48$& $0.48$\\
& Min& $0.31$& $0.31$& $0.32$& $0.31$& $0.31$& $0.32$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$\\
 & Max& $1.29$& $1.34$& $1.32$& $1.37$& $1.37$& $1.37$& $1.42$& $1.47$& $1.52$& $1.52$& $1.49$\\
\hline\\\\
$\textsc{HPIEF}$ & Mean & $1.60$& $1.62$& $1.63$& $1.66$& $1.67$& $1.68$& $1.70$& $1.70$& $1.73$& $1.75$& $1.77$\\
& Stdev & $1.29$& $1.32$& $1.33$& $1.36$& $1.37$& $1.38$& $1.41$& $1.41$& $1.43$& $1.46$& $1.48$\\
& Min& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$& $0.31$\\
 & Max& $3.22$& $3.22$& $3.29$& $3.39$& $3.40$& $3.44$& $3.60$& $3.52$& $3.57$& $3.70$& $3.77$\\
\hline\\\\
$\textsc{BnP-Poly}$ & Mean & $221.84$& $225.71$& $225.71$& $225.71$& $225.72$& $219.29$& $219.59$& $224.29$& $225.73$& $0.61$& $0.61$\\
& Stdev & $585.36$& $595.59$& $595.60$& $595.60$& $595.63$& $578.62$& $579.39$& $591.84$& $595.65$& $0.13$& $0.12$\\
& Min& $0.49$& $0.49$& $0.49$& $0.49$& $0.49$& $0.49$& $0.49$& $0.49$& $0.47$& $0.49$& $0.49$\\
 & Max& $1770.56$& $1801.49$& $1801.51$& $1801.51$& $1801.62$& $1750.18$& $1752.50$& $1790.15$& $1801.67$& $0.92$& $0.89$\\
\hline\\\\
$\textsc{CG-TSP}$ & Mean & $5.74$& $5.86$& $5.86$\\
& Stdev & $0.33$& $0.41$& $0.35$\\
& Min& $5.23$& $5.33$& $5.45$\\
 & Max& $6.26$& $6.50$& $6.48$\\
\hline\\\\
$\textsc{BnP-DFS}$ & Mean & $1.05$& $1.06$& $1.05$\\
& Stdev & $1.24$& $1.23$& $1.24$\\
& Min& $0.47$& $0.47$& $0.47$\\
 & Max& $4.30$& $4.27$& $4.30$\\
\hline\\\\
$\textsc{BnP-PICEF}$ & Mean & $5.97$& $3.66$& $5.77$& $6.12$& $55.11$& $12.35$& $16.02$& $21.79$& $37.32$& $45.26$& $54.44$\\
& Stdev & $13.50$& $6.43$& $10.47$& $7.59$& $130.10$& $8.16$& $5.10$& $6.77$& $26.52$& $19.67$& $12.69$\\
& Min& $0.72$& $0.99$& $1.49$& $2.49$& $4.82$& $7.31$& $11.69$& $16.73$& $22.50$& $30.92$& $43.52$\\
 & Max& $41.68$& $20.66$& $33.45$& $26.14$& $399.31$& $33.56$& $28.36$& $39.21$& $106.70$& $95.12$& $78.37$\\
\hline\\\\
\end{tabular}

\label{tbl:data}
\end{table}

==> sections/exp_tables/500pairs_0alts_mean.tex <==
\begin{table}[ht!bp]
\centering
\caption{$|P|~=~500,~|A|~=~0$}
\begin{tabular}
{ c r | r  | r  | r  | r  | r  | r  | r  | r  | r  | r  | r }
Method & & $L = 2$ & $L = 3$ & $L = 4$ & $L = 5$ & $L = 6$ & $L = 7$ & $L = 8$ & $L = 9$ & $L = 10$ & $L = 11$ & $L = 12$\\
\hline\\\\
$\textsc{PICEF}$ & Mean & $1.64$& $1.89$& $1.92$& $1.95$& $1.99$& $2.02$& $2.04$& $2.06$& $2.09$& $2.13$& $2.16$\\
& Stdev & $0.96$& $0.97$& $0.98$& $1.00$& $1.02$& $1.03$& $1.04$& $1.05$& $1.08$& $1.10$& $1.11$\\
& Min& $0.31$& $0.31$& $0.32$& $0.31$& $0.31$& $0.31$& $0.32$& $0.31$& $0.31$& $0.31$& $0.32$\\
 & Max& $3.19$& $3.22$& $3.24$& $3.27$& $3.32$& $3.32$& $3.40$& $3.40$& $3.47$& $3.52$& $3.52$\\
\hline\\\\
$\textsc{HPIEF}$ & Mean & $13.43$& $13.65$& $14.04$& $14.32$& $15.05$& $14.63$& $15.44$& $15.64$& $15.86$& $18.02$& $17.65$\\
& Stdev & $7.47$& $7.62$& $7.88$& $8.14$& $8.54$& $8.58$& $8.79$& $9.02$& $9.41$& $10.35$& $10.07$\\
& Min& $0.52$& $0.63$& $0.65$& $0.88$& $0.55$& $0.57$& $0.52$& $0.50$& $0.67$& $0.52$& $0.75$\\
 & Max& $18.51$& $19.89$& $20.44$& $22.74$& $22.34$& $23.67$& $22.80$& $23.45$& $25.14$& $27.21$& $27.27$\\
\hline\\\\
$\textsc{BnP-Poly}$ & Mean & $453.24$& $228.88$& $4.35$& $4.33$& $228.69$& $3.87$& $3.87$& $3.88$& $3.88$& $3.87$& $3.85$\\
& Stdev & $778.25$& $594.22$& $2.01$& $2.04$& $594.43$& $1.83$& $1.84$& $1.84$& $1.84$& $1.84$& $1.81$\\
& Min& $1.97$& $1.92$& $2.00$& $1.94$& $1.94$& $1.94$& $1.94$& $1.94$& $1.97$& $1.97$& $1.92$\\
 & Max& $1801.51$& $1801.02$& $7.58$& $7.66$& $1801.40$& $7.50$& $7.53$& $7.53$& $7.53$& $7.56$& $7.43$\\
\hline\\\\
$\textsc{BnP-DFS}$ & Mean & $234.89$& $234.89$& $234.89$& $234.90$& $234.90$& $234.96$& $234.87$& $234.89$& $234.95$& $234.92$& $234.89$\\
& Stdev & $592.19$& $592.19$& $592.18$& $592.19$& $592.18$& $592.16$& $592.19$& $592.18$& $592.16$& $592.17$& $592.18$\\
& Min& $3.32$& $3.32$& $3.32$& $3.32$& $3.32$& $3.32$& $3.30$& $3.32$& $3.32$& $3.30$& $3.30$\\
 & Max& $1801.45$& $1801.45$& $1801.46$& $1801.49$& $1801.45$& $1801.46$& $1801.44$& $1801.44$& $1801.44$& $1801.44$& $1801.44$\\
\hline\\\\
$\textsc{BnP-PICEF}$ & Mean & $17.47$& $489.05$& $241.64$& $251.10$& $474.24$& $479.78$& $541.92$& $387.22$& $413.45$& $467.99$& $642.82$\\
& Stdev & $22.81$& $763.33$& $591.10$& $588.83$& $754.91$& $713.01$& $761.69$& $620.36$& $561.11$& $534.46$& $530.38$\\
& Min& $3.22$& $4.30$& $7.56$& $14.32$& $29.66$& $54.63$& $88.38$& $119.65$& $156.95$& $224.51$& $307.77$\\
 & Max& $71.62$& $1804.37$& $1805.32$& $1808.25$& $1819.86$& $1896.86$& $1938.70$& $2027.37$& $1895.58$& $1879.92$& $1962.84$\\
\hline\\\\
\end{tabular}

\label{tbl:data}
\end{table}

==> sections/exp_tables/700pairs_0alts_mean.tex <==
\begin{table}[ht!bp]
\centering
\caption{$|P|~=~700,~|A|~=~0$}
\begin{tabular}
{ c r | r  | r  | r  | r  | r  | r  | r  | r  | r  | r  | r }
Method & & $L = 2$ & $L = 3$ & $L = 4$ & $L = 5$ & $L = 6$ & $L = 7$ & $L = 8$ & $L = 9$ & $L = 10$ & $L = 11$ & $L = 12$\\
\hline\\\\
$\textsc{BnP-Poly}$ & Mean & $455.47$& $455.54$& $455.69$& $455.78$& $455.74$& $455.79$& $455.75$& $455.71$& $455.75$& $455.69$& $455.73$\\
& Stdev & $778.26$& $778.17$& $778.13$& $778.29$& $778.09$& $778.04$& $778.11$& $778.13$& $778.11$& $778.17$& $778.30$\\
& Min& $4.32$& $4.32$& $4.35$& $4.40$& $4.48$& $4.40$& $4.50$& $4.67$& $4.53$& $4.71$& $4.60$\\
 & Max& $1804.00$& $1803.80$& $1803.94$& $1804.36$& $1803.81$& $1803.81$& $1803.89$& $1803.99$& $1803.99$& $1803.98$& $1804.53$\\
\hline\\\\
\end{tabular}

\label{tbl:data}
\end{table}

==> sections/relaxations.tex <==
In this section, we compare the linear-program relaxation (LPR) bounds of IP
formulations for kidney exchange. If $A$ and $B$ are two IP formulations for
kidney exchange, we write that $A$ \emph{dominates} $B$---or equivalently $Z_A
\prec Z_B$---to signify that for every problem instance, the LPR objective
value under $A$ is no greater than the LPR objective value under $B$, and that
for at least one instance it is strictly smaller. We write $A=B$ if the two
formulations have equal LPR objective values for every instance.

\subsection{Other IP formulations}

Before proceeding to the comparisons of LPR bounds, we review existing IP
formulations for kidney exchange. 

\subsubsection{Cycle formulation}\label{cf}

In the cycle formulation, a binary variable $z_c$ is used for each feasible
cycle or chain $c$ to represent whether it is selected in the solution. For
each vertex $v$, there is a constraint to ensure that $v$ is in at most
selected cycle or chain. Let $\cycles$ be the set of cycles in $D$ of length at
most $K$ and let $\chains$ be the set of NDD-initiated chains in $D$ of length
at most $L$. The model to be solved is as follows.

\begin{subequations}
\begin{align}
\max\ \sum_{c \in \cycles \cup \chains} w_cz_c & \label{eq:cf_objective}\\
\text{s.t. } \sum_{c \in \cycles \cup \chains : i \text{ appears in } c} z_c \leq 1 & \qquad i: 1 \leq i \leq |V| \label{eq:cf_a} \\
z_c \in \{0, 1\} & \qquad c \in \cycles \cup \chains \label{eq:cf_b}
\end{align}
\end{subequations}

Constraints (\ref{eq:cf_a}) ensure that the selected cycles and chains are
vertex disjoint.

\subsubsection{Edge formulation}\label{ef}

The edge formulation includes one variable for each edge in the directed graph. We consider here only the case of a pool with no NDDs. Let
\[
x_{ij} =
\begin{cases}
	1 & \text{if patient } j \text{ gets a kidney from donor } i \\
	0 & \text{otherwise}
\end{cases}
\]

The following IP is solved.
\begin{subequations}
\begin{align}
\text{Maximise} & \qquad \sum_{(i, j) \in A} w_{ij} x_{ij} & \label{eq:ef_objective}\\
\text{Subject to:} & \qquad \sum_{j: (j, i) \in A} x_{ji} = \sum_{j: (i, j) \in A} x_{ij} & 1 \leq i \leq n \label{eq:ef_a} \\
& \qquad \sum_{j: (i, j) \in A} x_{ij} \leq 1 & 1 \leq i \leq n \label{eq:ef_b} \\
& \qquad \sum_{1 \leq p \leq k} x_{i_p i_{p+1}} \leq k-1 & \text{paths } (i_1, i_2, \dots, i_k, i_{k+1}) \label{eq:ef_c} \\
& \qquad x_{ij} \in \{0, 1\} & (i, j) \in A \label{eq:cf_d}
\end{align}
\end{subequations}

Constraints (\ref{eq:ef_a}), the flow conservation constraints, ensure that
each vertex has aselected outgoing edge if and only if it has a selected
incoming edge. Constraints (\ref{eq:ef_b}), the capacity constraints, ensure
that each vertex has at most one outgoing arc. Constraints (\ref{eq:ef_c})
forbid long paths, in order to ensure that selected cycles have length at most
$K$.

The drawbacks of this formulation are that it has a weak linear-program
relaxation and an exponential number of constraints. As a result, the
formulation's run times compare unfavourably to the cycle formulation, even
when row generation is used to avoid keeping all constraints in
memory~\cite{Abraham07:Clearing}.

\subsubsection{Extended edge formulation}\label{eef}

In the extended edge formulation of Constantino et al. \cite{Constantino13:New},
several copies of $D$ are made, and at most one cycle may be chosen in each
copy. This avoids the need for the path constraints in the edge formulation
\ref{eq:ef_c}, and leads to a polynomial number of constraints.

\textbf{TODO: say more}

\subsubsection{TSP}

\textbf{TODO}

\subsubsection{SPLIT formulations (Mak-Hau)}

\textbf{TODO}


\subsection{LPR comparison of PIEF, PICEF, and cycle formulation}

\subsubsection{PIEF versus cycle formulation}

\input{relaxations/pief_vs_cf}

\subsubsection{PICEF versus cycle formulation}

\input{relaxations/picef_vs_cf}


\subsection{Ordering of formulations}

Tightness of relaxations are discussed in a few other
papers~\cite{Abraham07:Clearing,Constantino13:New,Anderson15:Finding}; we would like to fully
specify tightnesses relations over all formulations.  \textbf{Aim:} Have
rankings for the kidney exchange problem without chains and with chains.

PICEF dominates Edge Formulation by the k+1-cycle example from ABS-07.
CF dominates PICEF with chains by the two-arm example

With chains:
$$
\zEF{} \succeq \zEEF{} \succeq \zPICEF{} \succ \zCF{}
$$
\begin{itemize}
\item $\zEF{} \succ \zCF{}$~\cite{Abraham07:Clearing}
\item $\zEF{} \not\succ \zEEF{}$~\cite{Constantino13:New}
\item $\zEEF{} \not\succ \zEF{}$~\cite{Constantino13:New}
\item $\zEEF{} \succ \zCF{}$~\cite{Constantino13:New}
\item $\zPICEF{} \succ \zCF{}$~this paper, Theorem~\ref{thm:picef-vs-cf}
\item $\zEEF{} \succ \zPICEF{}$~this paper
\item $\zEF{} \succ \zTSP{}$~\cite{Anderson15:Finding}
\item Need to look at the other formulations in Ross' paper -- he has a subtour elimination and a cycle-ish formulation
\item Compare Ross' TSP vs PICEF -- Theorem~\ref{thm:tsp-vs-cf}
\item Klimentova vs CF -- I think they're the same?
\item Model 2, 6 of Mak-Hau?
\end{itemize}

Also how bad can PICEF vs CF get?

Without chains:
$$
\zEF{} \succeq \zEEF{} \succeq \zPIEF{} = \zTSP{} = \zCF{}
$$
\begin{itemize}
\item $\zEF{} \succeq \zCF{}$~\cite{Abraham07:Clearing}
\item $\zEF{} \not\succ \zEEF{}$~\cite{Constantino13:New}
\item $\zEEF{} \not\succ \zEF{}$~\cite{Constantino13:New}
\item $\zEEF{} \succ \zCF{}$~\cite{Constantino13:New}
\item $\zPIEF{} = \zCF{}$~this paper
\item $\zEEF{} \succeq \zPIEF{}$~this paper (same example as ABS-07)
\item $\zTSP{} = \zCF{}$ -- with only cycles the formulation is the ABS-07 formulation
\item Klimentova vs CF -- I think they're the same?
\item Model 2, 6 of Mak-Hau?
\end{itemize}

\input{sections/relaxations_temp_table}

\begin{theorem}\label{thm:tsp-vs-cf}
  $\zCF{} \prec \zTSP{}$ (with chains).
\end{theorem}
\begin{proof}
Need to show that any optimal solution to the LP relax of CF is also in the TSP polytope.

$\zCF{} \prec \zTSP{}$.  We now give a family of graphs for which $\zTSP{}$ is strictly greater than $\zCF{}$.

  \begin{figure}[ht!bp]
    \centering
    \input{figs/fig_tsp_proof}
    \caption{Family of graphs where $\zTSP{}$ is strictly looser than $\zCF{}$.}\label{fig:tsp_proof}
  \end{figure}

$a$ altruists, 1/a edge weights, 1 edge weights in a chain of length $a*L$, where $L$ is the chain cap.  No cycles so works for any cycle cap.
\end{proof}

\begin{theorem}\label{thm:split6-vs-ef}
  $\zSPLITSIX{} \prec \zEF{}$ (without chains).
\end{theorem}
\begin{proof}

($\zSPLITSIX{} \preceq \zEF{}$) This follows from the fact that when no NDDs
are present, SPLIT6 is equivalent to EF with additional constraints.

($\zSPLITSIX{} \prec \zEF{}$) Consider the graph in Figure
\ref{fig:splitsix_proof}, with edge weight equal to 1, and let $K=3$. The LPR
of EF has a feasible solution with objective value $10/3$: set
$z_{12}=z_{23}=z_{34}=z_{41}=2/3$ and $z_{13}=z_{31}=1/3$. \textbf{Can we show
that LPR of SPLIT6 can have max objective value 3?}

  \begin{figure}[ht!bp]
    \centering
    \input{figs/fig_split6_proof}
    \caption{A graph where $\zEF{}$ is strictly looser than $\zSPLITSIX{}$.}\label{fig:splitsix_proof}
  \end{figure}

\end{proof}



==> sections/relaxations_temp_table.tex <==
\begin{table}
\renewcommand{\arraystretch}{1.75}
{\color{blue}
\tbl{Comparison of LP relaxations, if NDD chains are used. Read row-name, table-entry, column-name. Don't add entries below main diagonal. (table to be replaced by DAG in paper)}{
\begin{tabular}{l|ccccccc}
               &  CF      &  EF      &  EEF                    & PICEF(=HPIEF?)                      &  TSP                             &SPLIT2       &SPLIT6        \\
CF             &  =       & $\prec$  & $\prec$                 & $\prec$ Thm.\ref{thm:picef-vs-cf}   & $\prec$ Thm.\ref{thm:tsp-vs-cf}  &             &              \\
EF             &          &  =       & $\not\prec$, $\not\succ$&                                     & $\succ$                          &             &              \\
EEF            &          &          &  =                      &                                     &                                  &             &              \\
PICEF(=HPIEF?) &          &          &                         &  =                                  &                                  &             &              \\
TSP            &          &          &                         &                                     &  =                               &             &              \\
SPLIT2         &          &          &                         &                                     &                                  &  =          &              \\ 
SPLIT6         &          &          &                         &                                     &                                  &             &  =           
\end{tabular}}
\label{tbl:comparison_with_chains}
}
\end{table}
\begin{table}
\renewcommand{\arraystretch}{1.75}
{\color{blue}
\tbl{Comparison of LP relaxations, if NDD chains are not used. Read row-name, table-entry, column-name. (table to be replaced by DAG in paper)}{
\begin{tabular}{l|cccc}
                   &  CF(=PIEF=TSP)   &  EF      &  EEF(=SPLIT2)           &SPLIT6        \\
CF(=PIEF=TSP)      &  =               & $\prec$  & $\prec$                 &              \\
EF                 &                  &  =       & $\not\prec$, $\not\succ$& $\succ$ Thm.\ref{thm:split6-vs-ef} ?     \\
EEF(=SPLIT2)       &                  &          &  =                      &              \\
SPLIT6             &                  &          &                         &  =          
\end{tabular}}
\label{tbl:comparison_without_chains}
}
\end{table}

